Sample, Scrutinize and Scale: Effective Inference-Time Search by Scaling Verification

Sampling-based search, a simple paradigm for utilizing test-time compute, involves generating multiple candidate responses and selecting the best one -- typically by having models self-verify each response for correctness. In this paper, we study the scaling trends governing sampling-based search. Among our findings is that simply scaling up a minimalist implementation of sampling-based search, using only random sampling and direct self-verification, provides a practical inference method that, for example, elevates the reasoning capabilities of Gemini v1.5 Pro above that of o1-Preview on popular benchmarks. We partially attribute the scalability of sampling-based search to a phenomenon of implicit scaling, where sampling a larger pool of responses in turn improves self-verification accuracy. We further identify two useful principles for improving self-verification capabilities with test-time compute: (1) comparing across responses provides helpful signals about the locations of errors and hallucinations, and (2) different model output styles are useful for different contexts -- chains of thought are useful for reasoning but harder to verify. We also find that, though accurate verification can be elicited, frontier models demonstrate remarkably weak out-of-box verification capabilities and introduce a benchmark to measure progress on these deficiencies.

==> search_arXiv/abstract.tex <==
\normalsize

Sampling-based search, a simple paradigm for utilizing test-time compute, involves generating multiple candidate responses and selecting the best one---typically by having models self-verify each response for correctness.
In this paper, we study the scaling trends governing sampling-based search.
Among our findings is that simply scaling up a minimalist implementation of sampling-based search, using only random sampling and direct self-verification, provides a practical inference method that, for example, elevates the reasoning capabilities of Gemini v1.5 Pro above that of o1-Preview on popular benchmarks.
We partially attribute the scalability of sampling-based search to a phenomenon of {\em implicit scaling}, where sampling a larger pool of responses in turn improves self-verification accuracy.
We further identify two useful principles for improving self-verification capabilities with test-time compute: (1) comparing across responses provides helpful signals about the locations of errors and hallucinations, and (2) different model output styles are useful for different contexts---chains of thought are useful for reasoning but harder to verify.
We also find that, though accurate verification can be elicited,  frontier models demonstrate remarkably weak out-of-box verification capabilities and introduce a benchmark to measure progress on these deficiencies.


==> search_arXiv/additional.tex <==
\subsection{Smaller Models}

\begin{table}[htbp]
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{AIME} & \textbf{MATH} & \textbf{LiveBench Math} & \textbf{LiveBench Reasoning} \\
\midrule
\multirow{3}{*}{Pro v1.5} 
& Pass@1 & 1 / 15 & 426 / 500 &  104 / 200 & 63 / 140 \\
& Consistency@200 & 4 / 15  & 460 / 500 & 118 / 200  & 75 / 140 \\
& Verification@200 & 8 / 15 & 467 / 500 & 135 / 200  & 97 / 140 \\
\midrule
\multirow{3}{*}{Flash v1.5} 
& Pass@1 & 2 / 15 & 407 / 500 &  96 / 200 & 65 / 140 \\
& Consistency@200 & 3 / 15  & 440 / 500 & 92 / 200  & 84 / 140 \\
& Verification@200 & 5 / 15 & 445 / 500 & 104 / 200  & 84 / 140 \\
\midrule
\multirow{1}{*}{Pro+Flash v1.5} 
& Verification@200 & 7 / 15 &  456 / 500 & 119 / 200  & 84 / 140 \\
\bottomrule
\end{tabular}
\begin{minipage}[t]{0.57\textwidth}
\vspace{0.6cm}
\centering
\includegraphics[width=\textwidth]{figs/gemini_comparison.png}
\end{minipage}
\hfill
\begin{minipage}[t]{0.38\textwidth}
\vspace{0.2cm}
\includegraphics[width=\textwidth]{figs/gemini_comparison2.png}
\end{minipage}
\caption{Accuracy rates with sampling-based search using either the Gemini v1.5 Pro model to both generate and verify responses (Pro), Gemini v1.5 Flash to both generate and verify responses (Flash), or Gemini v1.5 Pro model to generate responses and v1.5 Flash to verify responses (Pro+Flash). Verification@200 exceeds Consistency@200 for all model choices, while Pro+Flash Verification@200 matches or exceeds Pro Consistency@200.}
\label{tab:flash-sota}
\end{table}

\noindent
We also observe sampling-based search to be a powerful tool for enhancing smaller, lower-cost models.
Here, we apply sampling-based search to Gemini v1.5 Flash model, which has a nearly 20x lower inference cost than Gemini v1.5 Pro.
Table~\ref{tab:flash-sota} lists the performance of using the Flash model to evaluate candidate responses generated by the Pro model (Pro+Flash), and the performance of using the Flash model end-to-end for sampling-based search (Flash).
Sampling-based search still provides a significant improvement in performance for both Flash and Pro+Flash.
Moreover, Verification@200 still provides significant improvements over Consistency@200, albeit lesser in magnitude than for end-to-end use of Gemini Pro.
In addition, Flash Verification@200 using Gemini Flash is competitive with Pro Consistency@200, while Pro+Flash Verification@200 exceeds Pro Consistency@200.
We highlight that Pro+Flash Verification@200 has roughly the compute cost of Consistency@500---as our sampling-based search implementation is minimally optimized for efficiency, we expect costs to further decrease.


\subsection{Performance by Subtask}

\begin{table}[htbp]
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset} & \textbf{Cons@200} & \textbf{Verif@200} & \multicolumn{2}{c}{\textbf{Improvement (\%)}} & \textbf{Pass@200} & \textbf{\# Questions} \\
\cmidrule(r){4-5}
& & & \textbf{(Abs)} & \textbf{(Rel)} & & \\
\midrule
Berkeley MATH & 92.0\% & 93.4\% & 2\% $\uparrow$ & 20.0\% & 99.0\% & 500 \\
AIME 2024 & 26.7\% & 53.3\% & 100\% $\uparrow$ & 57.1\% & 73.3\% & 15 \\
Web-of-Lies-v2* & 75.5\% & 91.8\% & 22\% $\uparrow$ & 66.5\% & 100.0\% & 49 \\
Spatial* & 33.3\% & 46.7\% & 40\% $\uparrow$ & 21.5\% & 95.6\% & 45 \\
Zebra Puzzle* & 50.0\% & 67.4\% & 35\% $\uparrow$ & 36.4\% & 97.8\% & 46 \\
Competition\textsuperscript{\textdagger} & 66.2\% & 83.1\% & 26\% $\uparrow$ & 63.1\% & 93.0\% & 71 \\
AMPS Hard\textsuperscript{\textdagger} & 70.6\% & 77.7\% & 10\% $\uparrow$ & 33.5\% & 91.8\% & 85 \\
Olympiad\textsuperscript{\textdagger} & 25.0\% & 22.7\% & 9\% $\downarrow$ & -11.2\% & 45.5\% & 44 \\
\bottomrule
\end{tabular}

\caption{
The Pass@200, Consistency@200 (Cons@200), and Verification@200 (Verif@200) accuracy rates of the Gemini v1.5 Pro model using sampling-based search.
LiveBench Math\textsuperscript{\textdagger{}} and LiveBench Reasoning\textsuperscript{*} numbers are divided per task.
Absolute \% Increase (Abs) is the percentage improvement of Verification@200 over Consistency@200.
Relative \% Increase (Rel) is (Verification@200 - Consistency@200) / (Pass@200 - Consistency@200).
}
\label{tab:performance_metrics}
\end{table}

\noindent
The LiveBench benchmarks each consist of multiple subtasks.
In Table~\ref{tab:performance_metrics}, we break down the numbers reported in Table~\ref{tab:main-sota} for each of these subtasks.
We also provide in Table~\ref{tab:performance_metrics} the Pass@200 scores of the Gemini Pro model, which measure the probability that of 200 attempted responses to a question at least one is correct.
Pass@200 upper bounds what one can hope to achieve through Verification or Consistency.
Verification provides the greatest gains on AIME 2024, Web-of-Lies, Competition, and Zebra Puzzle.
In contrast, Verification does not improve on Consistency on the Olympiad task of the LiveBench Math benchmark.
We attribute this to the unique question design of LiveBench Olympiad task questions, which is incompatible with our implementation of Verification (see Appendix~\ref{app:oddity}).


==> search_arXiv/benchmark.tex <==
Frontier language models demonstrate a remarkable mismatch between their problem-solving capabilities and poor out-of-box verification capabilities.
These limitations have largely been attributed to the inability of current language models to self-diagnose hallucinations or enforce rigour \citep{zhang_how_2023,orgad_llms_2024,snyder_early_2024,kamoi_evaluating_2024, tyen_llms_2024, DBLP:conf/iclr/0009CMZYSZ24}.
However, our findings that models can be directed to accurately perform verifications at scale suggest that these out-of-box limitations can be addressed with standard methods like instruction tuning.
We compiled a set of challenging reasoning problems and candidate solutions to provide a benchmark for these deficits.

Each entry in this benchmark consists of a question, a correct candidate response, and an incorrect candidate response, and is manually curated from the residuals of our sampling-based search experiments (Section~\ref{section:pipeline}).
An example entry from this benchmark can be found below (see Appendix~\ref{app:examplebenchmark} for more).

\vspace{0.4cm}
\begin{tcolorbox}[title=Question from LiveBench Reasoning (Web-of-Lies Puzzle), breakable]
In this question, assume each person either always tells the truth or always lies. The person at the campground thinks their friend is lying. Mateo is at the aquarium. The person at the restaurant says the person at the hotel lies. Farid is at the movie theater. The person at the movie theater says the person at the campground lies. Ryan is at the shopping mall. The person at the cafe says the person at the campground lies. The person at the observatory says the person at the museum lies. The person at the museum says the person at the restaurant tells the truth. The person at the campground says the person at the airport tells the truth. The person at the campground tells the truth. Luna is at the restaurant. The person at the movie theater saw a firetruck. Isabella is at the observatory. The person at the amusement park says the person at the museum tells the truth. The person at the restaurant says the person at the shopping mall tells the truth. Liam is at the beach. Ayaan is at the airport. The person at the restaurant says the person at the beach tells the truth. Maya is at the amusement park. The person at the restaurant says the person at the aquarium lies. The person at the restaurant says the person at the movie theater lies. The person at the library says the person at the campground tells the truth. Elowen is at the hotel. Priya is at the library. The person at the gym says the person at the restaurant tells the truth. Kehinde is at the cafe. Anika is at the museum. Quan is at the campground. Soren is at the gym. Does the person at the museum tell the truth? Does the person at the restaurant tell the truth? Does the person at the movie theater tell the truth? Think step by step, and then put your answer in **bold** as a list of three words, yes or no (for example, **yes, no, yes**). If you don't know, guess.
\end{tcolorbox}
\definecolor{mydarkgreen}{rgb}{0.0, 0.5, 0.0} %


\begin{paracol}{2}

\switchcolumn[0]
\begin{tcolorbox}[breakable, colframe=mydarkgreen!70, colback=mydarkgreen!10, title=Correct response]
Here's how we can break down this logic puzzle:

1. **Quan is at the campground and tells the truth.** This is a given fact.

...

4. **The person at the restaurant (Luna) says the person at the hotel (Elowen) lies.**  We don't know yet if Luna is lying or telling the truth.

...

10. **Since Luna tells the truth about Farid, Luna *always* tells the truth.**  This unlocks several other pieces of information.

...

13. **The person at the cafe (Kehinde) says the person at the campground lies.** Since Quan tells the truth, Kehinde is lying.

Therefore:
* **Anika (museum):** Tells the truth.
* **Luna (restaurant):** Tells the truth.
* **Farid (movie theater):** Lies.

**yes, yes, no**
\end{tcolorbox}

\switchcolumn
\begin{tcolorbox}[breakable, colframe=red!70, colback=red!10, title=Incorrect Response Due to Hallucination]
Here's how we can solve this logic puzzle:

1. **Quan is at the campground and tells the truth.** This is given.

2. **The person at the airport (Ayaan) tells the truth.** Quan (campground) says the person at the airport tells the truth, and Quan tells the truth.

...

4. **Luna (restaurant) lies.**  The person at the restaurant says the person at the hotel (Elowen) lies. \textbf{\color{red} Later, the person at the restaurant says the person at the campground (Quan) lies.} Since Quan tells the truth, Luna (restaurant) must be lying.

...

Therefore:
* **Anika (museum): lies**
* **Luna (restaurant): lies**
* **Farid (movie theater): lies**

**Answer: no, no, no** 
\end{tcolorbox}
\end{paracol}

\noindent\begin{minipage}{\textwidth}
\captionof{figure}{Example of an entry in our verification benchmark. The question is sourced from the LiveBench Reasoning benchmark, and the two responses are generated by Gemini v1.5 Pro. The green response has the correct final answer; the red response has the wrong final answer due to hallucinating a non-existent clause.}
\label{fig:example}
\vspace{0.4cm}
\end{minipage}

\noindent
On each entry, our benchmark studies verification accuracy on two tasks:
\begin{enumerate}
    \item \textbf{Scoring task.} When given only the question and one of the responses, is the model able to discern the correctness of the response?
    \item \textbf{Comparison task.} When provided the whole tuple with the correctness labels of the responses masked and a guarantee that at least one response is correct, is the model able to discern which response is correct and which is incorrect?
\end{enumerate}

\noindent
The scoring task is also evaluated over a separate set of (question, response) pairs where the response reaches the correct final answer by coincidence but contains fatal errors and should be labeled by a reasonable verifier as being incorrect; an example can be found in Appendix~\ref{app:examplebenchmark}.
In the scoring task, models are provided only with the task description; in the comparison task, models are provided only with the task description and a suggestion to identify disagreements between responses in its reasoning.

Table~\ref{tab:benchmark} lists the baseline performances of current commercial model offerings on this benchmark.
Gemini v1.5 Pro is omitted from the benchmark as the entries in the benchmark are curated from the residuals of Gemini v1.5 Pro.
The prompts used in Table~\ref{tab:benchmark} are provided in Appendix~\ref{app:benchmarkprompts}.

As we previously observed, and has been noted in prior works \citep{tyen_llms_2024, kamoi_evaluating_2024}, verification errors are typically due to low recall.
Even the easier comparison task, models perform only marginally better---and often worse---than random chance.
In many cases, Consistency@5 performs worse than one-shot inference because Consistency simply averages out noise from an output distribution, meaning that a model biased towards producing an incorrect answer will do so with higher probability under Consistency.
Addressing these deficits in verification capabilities---which we see as low-hanging fruit for post-training---would enable not only better sampling-based search, but also other downstream applications of verification including reinforcement learning \citep[e.g.][]{o1-preview,deepseekai2025deepseekr1incentivizingreasoningcapability}, data flywheeling \citep[e.g.,][]{welleck_generating_2022}, and end-user experience (see Section~\ref{sec:related} for further discussion).


\begin{table}[htbp]
\centering
\begin{tabular}{llcccccc}
\toprule
\textbf{Model} & \textbf{Metric} & \multicolumn{3}{c}{\textbf{Scoring Accuracy}} & \multicolumn{1}{c}{\textbf{Comparison Accuracy}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-6}
 &  & \textbf{Correct} & \textbf{Wrong} & \textbf{Flawed} &  \\
\midrule
\multirow{2}{*}{GPT-4o} & Pass@1    & 76.5\%  & 31.0\% & 22.2\% & 43.2\%\\
 & Consistency@5 & 77.4\% & 30.0\% & 11.1\% & 35.4\% \\
\midrule
\multirow{2}{*}{Claude 3.5 Sonnet} & Pass@1 & 89.6\% & 22.5\% & 33.3\% & 56.1\% \\
 & Consistency@5 & 90.3\% & 17.5\% & 33.3\% & 61.2\% \\
\midrule
\multirow{2}{*}{o1-preview} & Pass@1 & 100\% & 68.8\% & 80.0\% & 84.5\% \\
 & Consistency@5 & 100\% & 79.4\% & 88.8\% & 92\% \\
\midrule
\multirow{2}{*}{Gemini 2.0 Flash} & Pass@1 & 73.5\% & 44.5\% & 60\% & 58\%  \\
 & Consistency@5 & 77.4\% & 42.5\% & 66.6\% & 58.7\% \\
\midrule
\multirow{2}{*}{Gemini 2.0 Thinking Flash} & Pass@1 & 75.4\% & 56.5\% & 53.3\%  & 80\%  \\
 & Consistency@5 & 77.4\%  & 55\% & 55.5\%  & 89.1\% \\
\midrule
\multicolumn{2}{c}{Random guessing}  & 80\% & 20\% & 20\% & 50\% \\
\bottomrule
\end{tabular}
\caption{Accuracy rates of commercial language models on our verification benchmark. For the task of response scoring (Scoring Accuracy), accuracy rates are broken down for entries that require identifying a correct response as being correct (Correct), entries that require identifying a wrong response as being wrong (Wrong), and entries that require identifying a wrong response that coincidentally reaches the correct answer as being wrong (Flawed).
GPT-4o and Claude 3.5 Sonnet only perform marginally better than random guessing across all tasks. o1-Preview performs better, but still fails to identify 20-30\% of wrong responses.
}
\label{tab:benchmark}
\end{table}


==> search_arXiv/conclusion.tex <==
This paper studied the scaling trends governing sampling-based search, finding that (1) it scales remarkably well even with simple implementations, (2) \emph{implicit scaling} plays a big role in this scalability, and (3) self-verification capability can be scaled with test-time compute using two key principles: comparisons localize errors, and responses should be rewritten for output style suitability.
To this end, we scaled a minimalist, embarrassingly parallel implementation of sampling-based search that, with sufficient test-time compute, is sufficient to attain state-of-art performance on a range of reasoning benchmarks.

Our results underscore the importance of the sampling-based search paradigm. 
Given that it complements other test-time compute scaling strategies, is parallelizable and allows for arbitrarily scaling, and admits simple implementations that are demonstrably effective, we expect sampling-based search to play a crucial role as language models are tasked with solving increasingly complex problems with increasingly large compute budgets.
We also see the performance of sampling-based search as providing both a strong baseline scaling trend that any non-trivial inference strategy should exceed, and a meaningful measure of a model's search capability when Pass@k is uninformative (e.g. on multiple choice exams).
We anticipate model self-verification capabilities to rapidly improve in the short term, as models learn to leverage the principles of implicit scaling and output style suitability, and drive improved scaling rates for sampling-based search.
Finally, our results also highlight the importance of being able to effectively sample massive and diverse sets of solutions for search.
This calls for more systematic inference alternatives to random sampling, such as agentic approaches that delegate search, and inference-aware optimization methods that maximize, e.g., Pass@k performance rather than Pass@1.


==> search_arXiv/details.tex <==
All experiments are run on Google Cloud with Gemini v1.5-Pro-002 and Gemini v1.5-Flash-002 models dated to September 2024.
Unless otherwise specified, the default parameters for our implementation of sampling-based search (Section~\ref{section:pipeline}) are $k_{\mathrm{inf}} = 200$, $\sigma_{\mathrm{inf}} = 1.5$, $k_{\mathrm{verif}} = 50$, $\sigma_{\mathrm{verif}} = 1$, and a maximum of 8,192 output tokens per query.
For all benchmarks, the scoring of candidate responses is performed using a language model rather than literal string comparison; details are in Appendix~\ref{app:scoring}.

\paragraph{Preliminary scoring.}
When generating $k_{\mathrm{verif}} = 50$ verification scores per candidate solution is too expensive, we first generate $k_{\mathrm{verif}} = 10$ preliminary verification scores and discard candidate solutions with an average score below $0.2$.
If a final answer is represented by more than 15 candidate responses, only the top 15--as measured by average preliminary score, tie-breaking randomly--are kept.
This results in a smaller pool of candidate solutions for which we compute all $k_{\mathrm{verif}} = 50$ verification scores.
Preliminary scoring is used on all datasets except AIME, which consists of 15 questions. 

\paragraph{Compute.}
On AIME, the verification process involves 32,000 
characters (roughly 13,000 tokens) of model output. %
Extrapolating from these figures, running the full sampling-based search pipeline on a question for $k_{\mathrm{inf}} = 200$ and $k_{\mathrm{verif}} = 50$ requires $200 \cdot 50 \cdot 13,000 \approx 130$M output tokens.
At around \$5/1M output tokens (public pricing of Gemini v1.5 Pro), this evaluates to approximately \$650 in cost.
Preliminary scoring reduces usage of output tokens by roughly 70\%, resulting in a per-question cost of \$200.
The use of Gemini Flash for verification further decreases cost to \$12 per question.

\paragraph{Datasets.}
Our MATH benchmark consists of 500 questions from the PRM800K \citep{DBLP:conf/iclr/LightmanKBEBLLS24} test split of Berkeley MATH \citep{DBLP:conf/nips/HendrycksBKABTS21}.
Our LiveBench Math benchmark consists of 200 randomly subsampled questions from the 368 available as of October 21st 2024, including AMC12 2023, AIME 2024, SMC 2023, USAMO 2023, IMO 2023, and synthetic math questions \citep{white2024livebenchchallengingcontaminationfreellm}.
Our LiveBench Reasoning benchmark consists of 140 questions from the 150 available as of October 21st 2024, including Zebra puzzles, Web-Of-Lies, and Spatial reasoning questions \citep{white2024livebenchchallengingcontaminationfreellm}.
Our AIME benchmark consists of the 15 questions in Exam II of AIME 2024 \citep{aime2024}. 


==> search_arXiv/intro.tex <==
Recent advances in language models highlight the importance of test-time compute scaling wherein one uses more compute during inference to enhance reasoning capabilities~\citep{o1-preview, deepseekai2025deepseekr1incentivizingreasoningcapability, agarwal2024manyshotincontextlearning, DBLP:conf/nips/Wei0SBIXCLZ22, DBLP:conf/nips/YaoYZS00N23, akyurek2024surprisingeffectivenesstesttimetraining}.
There are many methods for increasing test-time compute usage, including implicitly encouraging longer responses via reinforcement learning~\citep{o1-preview, deepseekai2025deepseekr1incentivizingreasoningcapability} or explicitly via prompting \citep{DBLP:conf/nips/Wei0SBIXCLZ22, DBLP:conf/nips/YaoYZS00N23}.
However, \emph{sampling-based search}---an instance of the generate-and-test approach where a model generates many responses in parallel, e.g. via random sampling or delegation, and selects what the model guesses to be the best one---remains one of the most natural and fundamental paradigms.
In addition to being complementary with other test-time compute scaling strategies, 
it also has the unique advantage of being embarrassingly parallel and allowing for arbitrarily scaling: simply sample more responses \citep{cobbe_training_2021,DBLP:conf/iclr/0002WSLCNCZ23}.
As a result, sampling-based search plays an increasingly crucial role as language models are set loose on frontier mathematical and scientific problems where inference compute budgets reach thousands of dollars or more per problem.

Though recent works demonstrate the benefits of sampling-based search \citep{cobbe_training_2021,DBLP:conf/iclr/0002WSLCNCZ23,xue_rcot_2023}, many questions remain as to what scaling trends govern this fundamental test-time compute scaling strategy.
To develop this understanding, we study a  minimalist---yet remarkably effective---instantiation of sampling-based search that uses a language model \citep{geminiteam2024gemini15unlockingmultimodal} to both generate a set of candidate responses via random sampling and select the best one by attempting to verify each response with natural language.
Specifically, we consider the case where models must self-verify their responses to  select the best answer, and do not make the strong assumption that one can access ground-truth answers or symbolic systems that exactly verify correctness.
In this setup, we address the question:
{\em what test-time scaling trends emerge as we scale both the number of sampled responses and verification capabilities?}
In particular, what are the limits of scaling this simple sampling-based search paradigm and how much does one need to continuously scale verification capability as one scales up search?

\paragraph{Our findings.}
We first identify scaling trends demonstrating that reasoning performance continues to improve with sampling-based search even as test-time compute is scaled well beyond the point where the performance of self-consistency~\citep{DBLP:conf/iclr/0002WSLCNCZ23} saturates.
At sufficient scale, even our minimalist implementation provides a significant leap in reasoning accuracy, lifting Gemini v1.5 Pro performance beyond o1-Preview, and Gemini v1.5 Flash beyond Gemini v1.5 Pro, on reasoning benchmarks such as LiveBench~\citep{white2024livebenchchallengingcontaminationfreellm} and the AIME~\citep{aime2024}, exhibiting sustained power-law scaling on the latter.
This not only highlights the importance of sampling-based search for scaling capability, but also suggests the utility of sampling-based search as a simple baseline on which to compare other test-time compute scaling strategies and measure genuine improvements in models' search capabilities.

We then attribute much of the strong scaling trends of sampling-based search to an \emph{implicit scaling} phenomenon.
Contrary to the intuition that sampling more responses should impose a greater burden on the verifier and reduce verification accuracy, we observe that scaling sampling indirectly enhances verification accuracy.
At a high-level, this is because well-written responses are easier to verify than poorly written responses, and scaling sampling widens the pool of well-written candidates.

We further identify two effective strategies for scaling verification capabilities using test-time compute: (1) directly comparing candidate responses and (2) task-specific rewriting of candidate responses.
The former mitigates a core weakness of language models, which struggle to identify mistakes and hallucinations unless given their locations~\citep{tyen_llms_2024}, by leveraging the fact that differences between candidate responses provide a strong signal for where errors might be located.
The latter leverages our observation of \emph{output style suitability} where chain-of-thought output formats are beneficial when generating responses but harder to verify than more formal, mathematically conventional writing styles.
Surprisingly, while effective verification can be easily elicited from frontier models by communicating these strategies, we observe that frontier models have remarkably poor out-of-box verification capabilities and introduce a new benchmark to quantify these deficits.


==> search_arXiv/overview.tex <==

\definecolor{subtleyellow}{RGB}{255, 255, 150}

\begin{table}[htbp]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \textbf{AIME} & \textbf{MATH} & \textbf{LiveBench Math} & \textbf{LiveBench Reasoning} \\
\midrule
Pass@1 & 1 / 15 & 426 / 500 &  104 / 200 & 63 / 140 \\
Consistency@200 & 4 / 15  & 460 / 500 & 118 / 200  & 75 / 140 \\
Consistency@1,000 & 3 / 15  & 460 / 500 & 120 / 200  & 73 / 140 \\
\rowcolor{subtleyellow} Verification@200 & {\textbf{8}} / 15 & \textbf{467} / 500 & \textbf{135} / 200  & \textbf{97} / 140 \\
o1-Preview@1 & 7 / 15 & 428 / 500 & 131 / 200  & 95 / 140 \\
\bottomrule
\end{tabular}
\caption{Accuracy rates of the Gemini v1.5 Pro model using sampling-based search (Verification@200) on reasoning benchmarks, compared to other inference methods and o1-Preview performance.
Verification@200 consistently improves on Consistency@200 and surpasses o1-Preview.\protect\footnotemark{}
Each score reflects a single run, due to the high expense of search at this scale (see Section~\ref{sec:tech}).
}
\label{tab:main-sota}
\end{table}

\footnotetext{The o1-preview-2024-09-12 numbers in Table~\ref{tab:main-sota} use publicly reported figures, with MATH and AIME figures sourced from the OpenAI blog post \citep{o1-preview}, and LiveBench figures sourced from the LiveBench leaderboard (\href{https://livebench.ai/}{livebench.ai}). We found the performance of o1-Preview as accessed through the OpenAI API to slightly differ with publicly reported figures, e.g. scoring 26\% not 44\% on AIME, and scoring 77\% not 67\% on LiveBench Reasoning.}

\paragraph{Preview and outline.}
Table~\ref{tab:main-sota} summarizes our first finding: that, with effective self-verification, simply scaling sampling-based search is sufficient to approach state-of-art performance on reasoning and math benchmarks (AIME 2024 \citep{aime2024}, LiveBench Math, LiveBench Reasoning \citep{white2024livebenchchallengingcontaminationfreellm}, and the Berkeley MATH dataset \citep{DBLP:conf/nips/HendrycksBKABTS21}).
It depicts the accuracy of the Gemini v1.5 Pro model \citep{geminiteam2024gemini15unlockingmultimodal} when only one solution\footnote{As we focus on answering reasoning problems, we use ``model responses'' and ``model solutions'' interchangeably.} is attempted per question (Pass@1), when 200 solutions are attempted and the most common final answer is selected (Consistency@200, \cite{DBLP:conf/iclr/0002WSLCNCZ23}), and under sampling-based search, when 200 solutions are attempted and scored for correctness with the highest scorer selected (Verification@200, Algorithm~\ref{alg:verification-pipeline}).
With sampling-based search (Verification@200), Gemini v1.5 surpasses the performance of o1-Preview, a model explicitly trained on reasoning problems to leverage significant test-time compute and perform internal search.

The rest of this paper is devoted to studying the three key factors behind the numbers in Table~\ref{tab:main-sota}.
Section~\ref{subsec:scaling} analyzes the remarkable scalability of sampling-based search, as one varies both the compute spent on search and verification;
Section~\ref{subsec:implicit} analyzes the phenomenon of \emph{implicit scaling} and its role in driving this scalability; and
Section~\ref{section:pipeline} discusses  important principles for scaling self-verification capability, which may be of independent interest.
We also highlight deficits in the verification capabilities of frontier models with a new benchmark in Section~\ref{sec:benchmark}.
Technical details and detailed discussion of related work are found in Sections~\ref{sec:tech} and \ref{sec:related} respectively.




\begin{algorithm}[htbp]
\caption{Sampling-Based Search (Verification@$k_{\mathrm{inf}}$)}
\label{alg:verification-pipeline}
\begin{algorithmic}[1]

\Require Prompt $Q$, language model $\mathrm{LM}$, scaling parameters $k_{\mathrm{inf}}, k_{\mathrm{verif}}, k_{\mathrm{tie}}$.

\State Populate $\mathcal{S}$ with $k_{\mathrm{inf}}$ samples from $\mathrm{LM}(``\mathrm{Answer} \;Q")$. \Comment{\textbf{Stage 1: Generate Responses}}

\For{each candidate response $s_i \in \mathcal{S}$}\Comment{\textbf{Stage 2: Verify Responses}}
    \State Populate $\mathcal{V}_i$ with $k_{\mathrm{verif}}$ samples from $\mathrm{LM}(``\mathrm{Return}\;1[\mathrm{response} \; s_i \; \mathrm{to} \;Q \;\mathrm{is \;correct}]")$.
\EndFor

\State Gather the highest-scored response  $\mathcal{S}_{\mathrm{Best}} = \{s_i \mid i \in [k_{\mathrm{inf}}], \mathrm{Avg}(\mathcal{V}_i) \geq \max_{j \in [k_{\mathrm{inf}}]} \mathrm{Avg}(\mathcal{V}_j) - 0.05\}$.

\If{$|\mathcal{S}_{\mathrm{Best}}| = 1$}
    \State Return response $s_{i^*}$ where $i^* = \max_{j \in [k_{\mathrm{inf}}]} \mathrm{Avg}(\mathcal{V}_j)$.
\Else
    \For{each pair of candidate responses $(s_i, s_j) \in \binom{\mathcal{S}_{\mathrm{Best}}}{2}$}\Comment{\textbf{Tie-Break: Compare Responses}}
    \State Populate $\mathcal{C}_{i,j}$ with $k_{\mathrm{tie}}$ samples from $\mathrm{LM}(``\mathrm{Which\;of\;responses\;}\{s_i, s_j\}\mathrm{\;to\;}Q\;\mathrm{is \;correct?}")$. 
    \EndFor
    \State Return response $s_{i^*}$ where $i^*$ is the winner of the most matchups $\{\mathcal{C}_{i,j} \mid s_i, s_j \in \mathcal{S}_{\mathrm{Best}}\}$.
\EndIf

\end{algorithmic}
\end{algorithm}


==> search_arXiv/related.tex <==
\paragraph{Test-time compute.}
Many of the recent advances in language model reasoning capabilities can be traced to increasing use of \textit{test-time compute}.
Inference strategies like chain-of-thought reasoning \citep{DBLP:conf/nips/Wei0SBIXCLZ22}, tree-of-thoughts \citep{DBLP:conf/nips/YaoYZS00N23} and self-critique  \citep{valmeekam2023largelanguagemodelsreally} result in improved reasoning performance at the cost of forming longer responses.
Reinforcement learning has emerged as a particularly successful strategy for effectively leveraging more test-time compute, wherein models learn from exploration to form lengthy chain-of-thought outputs that incorporate backtracking and search, despite not being explicitly taught to do so \citep{o1-preview, deepseekai2025deepseekr1incentivizingreasoningcapability}.
Inference-time model adaptation, whether through many-shot learning~\citep{agarwal2024manyshotincontextlearning, anil2024jailbreaking} or finetuning~\citep{akyurek2024surprisingeffectivenesstesttimetraining}, provides another avenue when training data is available.
We study sampling-based search: obtain a set of candidate responses from a model and apply an aggregation method to select a response, such as self-consistency/plurality voting \citep{DBLP:conf/iclr/0002WSLCNCZ23} or selecting a response with a reward/verifier model \citep{cobbe_training_2021}.
These various methods for scaling test-time compute are complementary; for example, sampling-based search can also be used on models trained to produce longer outputs.
We note that it is possible for models trained to produce long chains of thought to perform something resembling sampling-based search internally, in which case we still expect our observed scaling trends to hold.
However, we also expect explicit sampling-based search will remain indispensable, due to its greater parallelism and robustness than internally implemented search.

\paragraph{Scaling sampling-based search.}
The paradigm of sampling-based search provides three main knobs for scaling: generation, sampling, and selection.
While the cost of \emph{generating} each individual response can be scaled with previously mentioned interventions, such as chain-of-thought \citep[e.g.][]{DBLP:conf/nips/Wei0SBIXCLZ22}, reinforcement learning \citep[e.g.][]{o1-preview}, or inference-time adaptation \citep[e.g.][]{anil2024jailbreaking}, the cost of \emph{sampling} a set of responses can be scaled by increasing the number of responses generated~\citep{DBLP:conf/iclr/0002WSLCNCZ23,snell2024scalingllmtesttimecompute}.
We use random sampling to generate each set of candidate responses, which means the latter corresponds to simply taking more random draws.
However, this sampling can also be implemented in an agentic fashion, with a central model delegating the generation of responses so as to perform search more systematically.
The process of \emph{selecting} a response can be scaled by using more expensive rules: self-consistency provides a simple plurality voting rule at the lowest-cost end of the spectrum \citep{DBLP:conf/iclr/0002WSLCNCZ23}, while language model self-verification \citep[e.g.][see below]{xue_rcot_2023} and learned verification/reward models \citep[e.g.][see below]{cobbe_training_2021} provide a range of selection strategies that vary in cost and capability.
For more fine-grained control over the scaling of self-verification in our experiments, we apply plurality voting~\citep{DBLP:conf/iclr/0002WSLCNCZ23} to self-verification and vary our number of verification attempts per response.

\paragraph{Verification of language model outputs.}
A large body of recent work has studied the self-verification capabilities of large language models \citep[e.g.,][]{cobbe_training_2021,kadavath_language_2022,saunders_self-critiquing_2022,DBLP:conf/nips/KimBM23,DBLP:conf/nips/XieKZZKHX23,DBLP:conf/emnlp/WengZX0HLSLZ23,zhang_how_2023,xue_rcot_2023,li_making_2023,liu_large_2024,chow_inference-aware_2024,DBLP:conf/acl/JiangSYL0LK24,DBLP:conf/acl/DhuliawalaKXRLC24,snyder_early_2024,wu_large_2024,DBLP:conf/iclr/0009CMZYSZ24,kamoi_evaluating_2024,kamoi_when_2024,orgad_llms_2024,wen_language_2024,tyen_llms_2024,chen_simple_2024,kumar_training_2024,qu_recursive_2024,zhang_generative_2024,ko_real-time_2025,DBLP:conf/icml/HavrillaRNDZHR24}.
While some works---including ours---simply ask models to perform verification and parse the response, others have proposed custom methods of performing self-verification, including: recreating the problem from the response \citep{xue_rcot_2023,wu_large_2024}, masking and re-filling parts of the response \citep{DBLP:conf/emnlp/WengZX0HLSLZ23,DBLP:conf/acl/JiangSYL0LK24}, creating a rubric \citep{DBLP:conf/acl/DhuliawalaKXRLC24}, or asking models to choose from options \citep{DBLP:conf/nips/XieKZZKHX23,chen_simple_2024}.
Our work does not focus on optimizing for self-verification or advocate for any particular strategy.
However, in the course of performing our scaling study, we did identify several previously unstudied principles of self-verification that only arise at sufficiently large scale and may be of independent interest, including implicit scaling, output style suitability, and the importance of directly comparing responses.
Other related bodies of work study the learning of verifiers, often on top of a pretrained large language model~\citep[e.g.][]{cobbe_training_2021, saunders_self-critiquing_2022, li_making_2023, DBLP:conf/icml/HavrillaRNDZHR24, kumar_training_2024, qu_recursive_2024, chow_inference-aware_2024, zhang_generative_2024}, and the use of external tools for verification~\citep[e.g.][]{min_factscore_2023, gou_critic_2024, gao_embedding_2024,DBLP:conf/nips/KimBM23}.
We did not train customized verification models or permit verifier use of external tools in the listed experiments, as we found blackbox model access to be sufficient for effective verification at scale.
The limitations of model self-verification capabilities are also well-studied~\citep{kamoi_evaluating_2024, tyen_llms_2024, DBLP:conf/iclr/0009CMZYSZ24}, and can be remedied with external information \citep{DBLP:conf/iclr/0009CMZYSZ24} or hints for localizing errors \citep{tyen_llms_2024}.
Models especially struggle with self-diagnosing hallucinations \citep{zhang_how_2023,orgad_llms_2024,snyder_early_2024}, despite awareness of their own limitations \citep{kadavath_language_2022}, and are often incentivized to obfuscate errors \citep{wen_language_2024}.

\paragraph{Applications of verification.}
In addition to being used to select from candidate responses~\citep{cobbe_training_2021,li_making_2023,DBLP:conf/emnlp/WengZX0HLSLZ23,DBLP:conf/acl/JiangSYL0LK24,chen_simple_2024,DBLP:conf/nips/XieKZZKHX23}, verifiers can be used to guide iterative improvements to a model's output by providing feedback to the generating model~\citep{DBLP:conf/nips/KimBM23,xue_rcot_2023,valmeekam2023largelanguagemodelsreally,wu_large_2024,DBLP:conf/iclr/0009CMZYSZ24,DBLP:conf/acl/DhuliawalaKXRLC24, stechly2024chainthoughtlessnessanalysiscot, stechly2024selfverificationlimitationslargelanguage,qu_recursive_2024,DBLP:conf/icml/HavrillaRNDZHR24,ko_real-time_2025}. 
Another important application of verification is in enhancing model capabilities.
For example, verification results for model outputs can be fed back into models as feedback via in-context reinforcement learning~\citep{shinn_reflexion_2023}, reinforcement learning~\citep{uesato_solving_2022,peng_check_2023,madaan_self-refine_2023,kumar_training_2024, chow_inference-aware_2024}, or finetuning~\citep{ welleck_generating_2022,paul_refiner_2024,an_learning_2024,DBLP:journals/tmlr/SinghCAAPGLH0XP24}, in an approach known as data flywheeling.
Verification has also been explored as a means of encouraging models to produce better written responses~\citep{anil_learning_2021,kirchner2024proververifiergamesimprovelegibility}.
From a product perspective, verification capabilities are also important to the workflow of end users \citep{collins_evaluating_nodate}.


==> search_arXiv/scaling.tex <==
This section examines how reasoning capability scales with two fundamental test-time compute axes:

\begin{itemize}[label=$\bullet$, left=0.1cm]
    \item \textbf{Search} refers to the compute used to discover candidate solutions. In this section, our knob for scaling search is the number of responses sampled for each reasoning problem ($k_{\mathrm{inf}}$ in Algorithm~\ref{alg:verification-pipeline}). %
    \item \textbf{Verification} refers to the compute used to scrutinize candidate solutions. Our knob for scaling verification is the number of verification scores we compute and average over per solution ($k_{\mathrm{verif}}$). %
\end{itemize}
For computational reasons, this section uses a streamlined form of Algorithm~\ref{alg:verification-pipeline} that omits tie-breaking. This, for example, results in significant underestimates of Verification@k on MATH (see Table~\ref{tab:ablation}). All figures are averaged over 20 random seeds, where each run subsamples solutions and verification scores from a primary run that sampled 200 solutions per question and 50 verification scores per solution.

\subsection{Scaling Trends}
\label{subsec:scaling}

\begin{figure}[tbp]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/AIME_absolute.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/MATH_absolute.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/LiveBenchMath_absolute.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/LiveBenchReasoning_absolute.png}
    \end{subfigure}

    \caption{Heatmap of Gemini v1.5 Pro accuracy rates using sampling-based search (without tie-breaking) as the number of responses generated (x-axis) and verification attempts (y-axis) increase.
    Warmer colors indicate higher accuracy (cubic scale).
    The largest gains occur when scaling both search and verification, with the strongest trend on AIME.
    }
    \label{fig:four_images}
\end{figure}

Figure~\ref{fig:four_images} provides a heatmap of Verification@k on each benchmark in Table~\ref{tab:main-sota}  as we scale search and verification.
In addition to clear burn-in costs along both axes of scale, we can observe that the largest performance gains are realized when search and verification are both scaled.
These trends also indicate that the performances of sampling-based search, as reported in Table~\ref{tab:main-sota}, have not yet been scaled to saturation on these benchmarks.
This scaling trend is strongest on the AIME benchmark, where performance is bottlenecked by $k$ (search); we attribute this bottleneck to the difficulty of the AIME questions resulting in correct solutions only appearing with very low probability (see Table~\ref{tab:verifscores}).

\subsection{Implicit Scaling}
\label{subsec:implicit}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\textwidth]{figs/side_by_side_plots.png}
    \caption{
    Plot of Gemini v1.5 Pro accuracy rates using sampling-based search (without tie-breaking and with $k_{\mathrm{verif}} = 50$) on \emph{ambiguous questions only} as the number of responses generated increases.
    A question is ambiguous when the model generates at least one candidate response with a correct final answer.
    Accuracy on ambiguous questions increases with search.}
    \label{fig:four_images_norm2}
\end{figure}

Scaling sampling-based search along the \emph{search} axis by sampling more solutions, i.e. increasing $k$, should have two effects on performance that partially cancel out: (1) the verifier must discriminate between more solutions, increasing the likelihood of error and (2) the generator is more likely to produce at least one solution that reaches a correct final answer, i.e. Pass@k increases.

\begin{figure}[htbp] %
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
    \hfill
        \includegraphics[width=0.9\textwidth]{figs/AIME_relative.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/LiveBenchReasoning_relative.png}
    \hfill
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
    \hfill
        \includegraphics[width=0.9\textwidth]{figs/LiveBenchMath_relative.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figs/MATH_relative.png}
    \hfill
    \end{subfigure}
    
    \caption{
    Heatmap of Gemini v1.5 Pro accuracy rates using sampling-based search (without tie-breaking) on \emph{ambiguous questions only} as the number of responses generated (x-axis) and verification attempts (y-axis) increase.
    Warmer colors indicate higher accuracy (linear scale).
    A question is ambiguous when the model generates at least one candidate response with a correct final answer.
    Accuracy on ambiguous questions increases with search (x-axis).
    }
    \label{fig:four_images_norm}
\end{figure}
To isolate the first effect, we study the model's Verification@k accuracy on ``ambiguous'' questions: questions where at least one of the model’s \(k\) candidate solutions reaches the correct final answer (note that Pass@k equals the number of ambiguous questions).
Figure~\ref{fig:four_images_norm2} and Figure~\ref{fig:four_images_norm} do exactly this, plotting Verification@k accuracy measured only on ambiguous questions from each benchmark.
To reduce noise in these figures, we deterministically omit benchmark questions that Consistency@200 answers correctly or where, with high probability, 50 random responses result in either all correct or all incorrect final answers.

After controlling for the growth of Pass@k, we should expect a trend of decreasing accuracy if we increase $k$ but keep the number of verification attempts constant.
However, Figure~\ref{fig:four_images_norm2} shows the reverse trend: accuracy increases with $k$.
This demonstrates an \emph{implicit scaling} of verification accuracy, where increasing the number of generated responses increases not only the chance that at least one response is correct (Pass@k) but also the chance that at least one of the correct responses is of higher quality.
Here, quality can be understood as the rigour or flawlessness of a response; a lower quality solution may be generally correct but fail to justify a non-trivial step or err in a non-critical step of its reasoning.

Implicit scaling suggests that verification should become more accurate, and sampling-based search should become more effective, with the use of more capable base models that produce more sound reasoning and compelling proofs of correctness.
Because the number of ambiguous questions strictly increases with more candidate solutions, the implicit scaling effect also explains the overall accuracy scaling gains in Figure~\ref{fig:four_images}: larger $k$ increases both the number of ambiguous questions (Pass@k) and accuracy on the set of ambiguous questions.

\subsection{The Long Tail of Response Distributions}
\label{subsec:tail}

\begin{figure}[htbp] %
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/AIME_lines.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/MATH_lines.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/LiveBenchMath_lines.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/LiveBenchReasoning_lines.png}
    \end{subfigure}

    \caption{Line graph depicting the accuracy rates of the Gemini v1.5 Pro model using sampling-based search as the number of candidate responses generated is scaled upwards.
    The number of verification attempts is fixed at 50 for all plots.
    The depicted accuracies are obtained without tie-breaking and may be lower than reported elsewhere.
    Verification@k improves with $k$ even when Consistency@k stagnates on AIME and LiveBench Reasoning.
    }
    \label{fig:four_images2}
\end{figure}

\noindent
We can directly observe Verification@k scaling beyond the saturation point of Consistency@k in Figure~\ref{fig:four_images2}, where we plot their performance after fixing the number of verification attempts at 50.
On AIME, the most technically challenging benchmark, Verification@k demonstrates power law scaling even as Consistency@k begins to plateau.
The rapid saturation of Consistency@k can be attributed to the fact that, while it is effective at small scales in averaging out noisy mistakes, it necessarily plateaus as it converges on the most probable response;  for example, Consistency@50 has the same accuracy as Consistency@10,000 on AIME.
Consider cheaply sampling a vast set of solutions from a weak but ergodic model: Consistency@k is unlikely to return a correct solution, but an effective verifier should still be expected to detect rare but correct solutions in the long-tail of the response distribution.
We find an example of this on the AIME 2024 exam, where the Gemini v1.5 model struggles to identify the correct answer to Problem 11 on Exam II.
Table~\ref{tab:verifscores} shows the final answers from 200 randomly sampled Gemini v1.5 solutions, of which only one is correct (``601,'' in green).
Consistency returns the incorrect answer of ``1'' (in red), which appears in over half the responses. In contrast, Verification successfully identifies the solution reaching the correct answer from the response distribution's long-tail, assigning a $\le$36\% score to each solution reaching a final answer of ``1'' but a 98\% score to the single solution reaching ``601''.
\begin{table}[htbp] %
\centering
\begin{minipage}[t]{0.42\textwidth}
\vspace{0pt}
\begin{tcolorbox}[title={Problem 11, AIME 2024}]
\raggedright
    Find the number of triples of nonnegative integers $(a, b, c)$ satisfying $a + b + c = 300$ and $a^2 b + a^2 c + b^2 a + b^2 c + c^2 a + c^2 b = 6,000,000$.
\end{tcolorbox}

\includegraphics[width=\textwidth]{figs/longtail.png}
\end{minipage}
\hfill
\begin{minipage}[t]{0.56\textwidth}
\vspace{0pt}
\begin{tabular}{cccc}
\toprule
\textbf{Verification Score} & \multicolumn{2}{c}{\textbf{Final Answer}} & \textbf{\# Solutions} \\
\midrule
\rowcolor{green}
0.98 & 601    & (Correct) & \textbf{1}   \\
0.76 & 6      & (Wrong)   & 11  \\
0.52 & 0      & (Wrong)   & 14  \\
0.40 & 7      & (Wrong)   & 21  \\
0.38 & 4      & (Wrong)   & 10  \\
\rowcolor{red} 0.36 & 1      & (Wrong)   & \textbf{124} \\
0.22 & 10     & (Wrong)   & 2   \\
0.20 & 3      & (Wrong)   & 9   \\
0.18 & 301    & (Wrong)   & 1   \\
0.16 & 45451  & (Wrong)   & 1   \\
0.14 & 101    & (Wrong)   & 2   \\
0.06 & 2      & (Wrong)   & 1   \\
0.04 & 45151  & (Wrong)   & 1   \\
0.04 & 303    & (Wrong)   & 1   \\
0.00 & 100    & (Wrong)   & 1   \\
\bottomrule
\end{tabular}
\end{minipage}

\raggedright
\caption{The final answers identified by the Gemini v1.5 Pro model to Problem 11 on AIME 2024, sorted by verification score and annotated with their multiplicity in 200 solution generations.
The correct final answer (green) is only found by 1 generated response whereas Consistency@200 selects an incorrect final answer (red) that is found by 124 generated responses.} %
\label{tab:verifscores}
\end{table}
Scaling verification capability is key to driving improved search, allowing for discerning between answers that appear correct with 98\% vs. 76\% confidence.
The fact that verification can be used to so effectively leverage the long-tail of model response distributions also suggests that Pass@k, not Pass@1, should be the key performance metric for search applications.
Existing post-training techniques (e.g., reinforcement learning from human feedback (RLHF) \citep{DBLP:conf/nips/Ouyang0JAWMZASR22}) which explicitly optimize for Pass@1 may potentially be doing so at the expense of Pass@k and inhibiting search capability.


==> search_arXiv/verif.tex <==
\noindent
In the process of scaling sampling-based search, we identified two general principles for eliciting more accurate language model self-verification, that may be of independent interest.
\begin{enumerate}
    \item \emph{Compare responses to localize errors.} 
    Disagreements between candidate solutions strongly signal the potential locations of their errors.
    This can be leveraged to combat the fact that language models have low recall (i.e., often overlook) when asked to identify mistakes and hallucinations \citep{tyen_llms_2024,kamoi_evaluating_2024}, as models are able to identify errors when provided their locations  \citep{tyen_llms_2024}.
    Specifically, we can improve the self-verification of a candidate response by providing the verifier with other responses to compare the candidate against---an instance of implicit scaling.

    \item \emph{Rewrite responses for output style suitability.}
    The optimal output style of a language model should depend on the task.
    Writing in a linear chain of thought--- which includes detailing reasoning before committing to a claim---is effective when generating responses (search) \citep{DBLP:conf/nips/Wei0SBIXCLZ22}.
    However, responses are easier to verify when written rigorously, hierarchically, and modularly.
    This can be leveraged by having verifiers first rewrite candidate responses in, e.g., an expanded mathematically conventional theorem-lemma-proof format rather than directly evaluating chains-of-thought.
\end{enumerate}

\noindent
These principles also provide levers for scaling self-verification capability with test-time compute, including by (1) sampling and providing verifiers with more responses to compare between and (2) rewriting responses with increasing rigour and structure.

\subsection{Sampling-Based Search Implementation}
We now detail our minimalist implementation of sampling-based search (summarized in Algorithm~\ref{alg:verification-pipeline}) that uses only parallelizable blackbox queries to a language model.
It generates candidate responses by randomly sampling from models and select responses by asking models to self-verify; prompts are identical across all benchmarks and provided in the source code.

\paragraph{Step 1: Generate Candidate Responses.}
A language model generates $k_{\mathrm{inf}}$ candidate responses (candidate solutions) in parallel to each question, using temperature $\sigma_{\mathrm{inf}}$.

\paragraph{Step 2: Verify Candidate Responses.}
A language model generates $k_{\mathrm{verif}}$ binary ``verification scores'' for each candidate in parallel, indicating whether its final answer is correct.
Each scoring attempt is a single conversation thread that rewrites the response as a theorem, supporting lemmas, and proofs (examples in Appendix~\ref{app:rewrite}) and systematically scans for errors.
The highest scoring response is selected.

\paragraph{Tie-Break: Compare Candidate Responses.}
When the three highest scoring candidates score within 5\% of one another and disagree on the final answer, a language model directly compares the responses in pairwise matchups.
Each matchup is a single conversation thread that identifies where responses diverge and, at each such point, determines which side is correct.
Each matchup is repeated \(k_{\mathrm{tie}} = 100\) times.
The response with the most wins in the round-robin tournament is selected.

\subsection{Ablation Studies}
We can individually ablate the practices of comparing and rewriting candidate responses to confirm their role in eliciting greater verification capability.

\paragraph{Ablating comparisons.}
The step of asking models to directly compare candidate solutions with similar verification scores significantly increases sampling-based search performance.
This is demonstrated in Table~\ref{tab:ablation}, where we depict the accuracy rates from Table~\ref{tab:main-sota} alongside the accuracy rates after ablating the tie-breaking step.
These comparisons have the greatest impact when models struggle from low recall and excessively assign high verification scores.
On the MATH benchmark, which sees the greatest lift from comparisons, the average verification score of the top 3 candidate responses is nearly 90\%.
Recall that, as a result, the figures reported in Section~\ref{sec:allscaling} that omit tiebreaking significantly underestimate sampling-based search performances (Verification@k).

\begin{table}[htbp]
\centering
\begin{minipage}[c]{0.68\textwidth}
\vspace{0cm}
\begin{tabular}{lccccc}
\toprule
\textbf{Dataset} & \textbf{Cons@200} & \multicolumn{2}{c}{\textbf{Verification@200}} \\
                 &                   & \textbf{Without} & \textbf{With Tie-Break} \\
\midrule
MATH              & {460} / {500}   & {457} / {500}   & {467} / {500} \\
LiveBench Math        & {118} / {200}   & {125} / {200}   & {135} / {200} \\
LiveBench Reasoning & {75} / {140}    & {94} / {140}    & {97} / {140} \\
AIME              & {4} / {14}      & {7} / {14}      & {8} / {14}   \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[c]{0.31\textwidth}
\vspace{0cm}
\includegraphics[width=\textwidth]{figs/tiebreak.png}
\end{minipage}

\caption{Accuracy rates of Gemini v1.5 Pro using sampling-based search, with and without tie-breaking.
Tie-breaking provides most of Verification@200's gains on Consistency@200 (Cons@200) on MATH and LiveBench Math, and smaller gains on AIME and LiveBench Reasoning.
}
\label{tab:ablation}
\end{table}


\paragraph{Ablating rewritings.}
We explored a limited number of prompts for self-verification, including prompts which omit instructing the model to rewrite responses.
We did not perform further prompt optimization and expect refinements would boost accuracy.
Table~\ref{tab:prompt_tuning_results} shows each prompt’s probability of mislabeling correct solutions (false positive) and incorrect solutions (false negative), with the former generally having a more severe impact on downstream performance.
We evaluated these prompts on 1,080 candidate responses to 54 level-5 questions from the MATH training split, and 120 candidate responses to 6 questions from AIME 2023.
A response is marked as incorrect if, of 20 verification attempts, the number finding an error in the solution exceeds the equal error rate threshold.


\emph{Main} refers to manually written prompts used in our experiments.
\emph{Shortened} refers to a shorter variant of ``Main'' that omits, e.g., instructions to avoid truncation.
\emph{Without Rewrite} refers to a variant of ``Main'' that omits instructing the verifier to first rewrite responses.
\emph{Split-Context} refers to a variant of ``Main'' that creates separate conversation threads to individually verify pieces of the response.

The gap between the performance of ``Main'' and ``Without Rewrite'' demonstrates that ablating the rewriting of solutions negatively impacts verification performance. Similarly, the gap with ``Split-Context'' demonstrates that splitting the verification process into separate conversation threads sharply decreases performance due to low precision, which we attribute to miscalibration.

\begin{table}[htbp]
\centering
    \hfill
\begin{minipage}[t]{0.5\textwidth}
\vspace{0.4cm}
    \begin{tabular}{lcc|cc}
        \toprule
        \textbf{Prompt Style} & \multicolumn{2}{c}{\textbf{MATH}} & \multicolumn{2}{c}{\textbf{AIME}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & \textbf{FPR} & \textbf{FNR} & \textbf{FPR} & \textbf{FNR} \\
        \midrule
        Main            & 14\% & 17\% & 7\%  & 7\%  \\
        Shortened     & 17\% & 17\% & 7\%  & 7\%  \\
        Without Rewrite & 16\% & 18\% & 11\% & 12\% \\
        Split-Context   & 19\% & 23\% & 11\% & 14\% \\
        \bottomrule
    \end{tabular}
    \end{minipage}
    \hfill
\begin{minipage}[t]{0.45\textwidth}
\vspace{0cm}
\includegraphics[width=\textwidth]{figs/overlapping_circles.png}
\end{minipage}
    \caption{Verification scoring accuracy rates of the Gemini v1.5 Pro model for various prompts. False positive rate (FPR) refers to how often a correct response is labeled as incorrect; false negative rate (FNR) refers to how often an incorrect response is labeled as correct. %
    }
    \label{tab:prompt_tuning_results}
\end{table}

